Socially Aware Bias Measurements for Hindi Language Representations

Language representations are efficient tools used across NLP applications, but they are strife with encoded societal biases. These biases are studied extensively, but with a primary focus on English language representations and biases common in the context of Western society. In this work, we investigate biases present in Hindi language representations with focuses on caste and religion-associated biases. We demonstrate how biases are unique to specific language representations based on the history and culture of the region they are widely spoken in, and how the same societal bias (such as binary gender-associated biases) is encoded by different words and text spans across languages. The discoveries of our work highlight the necessity of culture awareness and linguistic artifacts when modeling language representations, in order to better understand the encoded biases.

==> gender_in_hindi.tex <==







==> survey.tex <==
%\subsection{Fairness in Global NLP}
%Fairness of language models is of great importance and has seen a lot of work in the recent times. The work however is mostly focused on English language and Western perspectives of societal biases. Work related to fair NLP in other languages which represent a culture with different biases has not been investigated as widely. We survey here some of the notable work.
%Although various works have been put forwards in bias mitigation and detection for English language, a little work has been performed upon other languages too.
Some notable work does tackle the challenges of societal biases in language representations coming from different cultures and languages apart from English.
\citet{lauscher-etal-2020-araweat} study different forms of biases in dialect specific Arabic word embeddings (CBOW and FastText). They  %perform diachronic analyses over different time periods of corpora and 
detect bias using both explicit and implicit bias detection methods like WEAT~\cite{caliskan2017semantics} and  K-means++. %and analyze differences in societal biases across the modern Arabic dialect and Egyptian Arabic dialect.
 \citet{chavez-mulsa-spanakis-2020-evaluating} demonstrate gender bias in Dutch language representations(FastText and contextual BERTJe) using tests like WEAT and further, adapt hard debiasing~\cite{bolukbasi2016man} to mitigate biases.
\citet{kurpicz2020cultural} identify that there is a bias towards gender and origin in both German and French word embeddings by creating new tests for the languages using domain knowledge.
\citet{zhou-etal-2019-examining} study gender bias in languages with grammatical gender like Spanish and French and extend existing approaches to mitigate gender bias in their word embeddings under both monolingual and bilingual settings. %Their experiments on modified Word Embedding Association Test, word similarity, word translation, and word pair translation tasks show that the proposed approaches can effectively reduce the gender bias while preserving the utility of the original embeddings.
%Biases in Hindi has also seen limited work with the most notable being that of
\citet{10.1145/3377713.3377792} explore adaptation of bias detection and mitigation in Hindi language representations. Their work however is restricted to only binary gender bias and not the other cultural biases dominant in the Indian society. They too adapt hard debiasing to mitigate biases by making a small set of gender definition words in Hindi and using them to find the gender subspace. %Unlike previous approaches they use k-means clustering to extract the latent gender direction. However,
However, the grammatically gendered nature of Hindi as compared to English is not considered.

In this work, we (i) discuss the gendered nature of Hindi and the implications on bias detection and mitigation techniques,
(ii) adapt methods of bias detection to Hindi and demonstrate how translation is not sufficient,
(iii) adapt methods of debiasing gender bias keeping in mind the different rich gendered information to be retained, and (iv) highlight the other societal biases dominant in Hindi representations and ways to detect and mitigate them.

%They train an SVM classifier that predicts whether a gender neutral word is gender-neutral or not. In order to debias the static word embeddings, gender subspace/direction was determined by conducting PCA over gendered word pairs. The embeddings are debiased by making the word embeddings orthogonal to the gender subspace. However, the types of biases specific to the cultural aspect of Hindi language is not considered. Bias detection is done by an SVM model which is trained upon biased embeddings and hence it is inherently biased. In addition, mitigation of gender bias is not explored from the perspective of gendered nature of Hindi grammar.


